MedLSAM: Localize and Segment Anything Model for 3D CT Images

Recent advancements in foundation models have shown significant potential in medical image analysis. However, there is still a gap in models specifically designed for medical image localization. To address this, we introduce MedLAM, a 3D medical foundation localization model that accurately identifies any anatomical part within the body using only a few template scans. MedLAM employs two self-supervision tasks: unified anatomical mapping (UAM) and multi-scale similarity (MSS) across a comprehensive dataset of 14,012 CT scans. Furthermore, we developed MedLSAM by integrating MedLAM with the Segment Anything Model (SAM). This innovative framework requires extreme point annotations across three directions on several templates to enable MedLAM to locate the target anatomical structure in the image, with SAM performing the segmentation. It significantly reduces the amount of manual annotation required by SAM in 3D medical imaging scenarios. We conducted extensive experiments on two 3D datasets covering 38 distinct organs. Our findings are twofold: 1) MedLAM can directly localize anatomical structures using just a few template scans, achieving performance comparable to fully supervised models; 2) MedLSAM closely matches the performance of SAM and its specialized medical adaptations with manual prompts, while minimizing the need for extensive point annotations across the entire dataset. Moreover, MedLAM has the potential to be seamlessly integrated with future 3D SAM models, paving the way for enhanced segmentation performance. Our code is public at \href{https://github.com/openmedlab/MedLSAM}

==> tabel/structseg.tex <==
\begin{table*}[!h]
\caption{DSC (mean$\pm$std \%) evaluation of 3D head-and-neck organs segmentation in the StructSeg Task1 dataset. The table compares the performance of SAM and MedSAM as a segmentation basis within the MedLsAM framework, along with results from manually assisted localizations.}
\centering
\scalebox{1}{
\begin{tabular}{c|cc|cc} \hline
Localization & \multicolumn{2}{c|}{MedLAM} & \multicolumn{2}{c}{Manual} \\ \cline{1-5}
Organs & SAM & MedSAM & SAM & MedSAM\\\hline
Brain Stem & 53.5 $\pm$ 5.5 & \textbf{64.7 $\pm$ 6.3} & 65.2 $\pm$ 3.7 & \textbf{72.8 $\pm$ 3.3} \\
Eye L & \textbf{63.9 $\pm$ 6.1} & 61.1 $\pm$ 6.1 & \textbf{67.6 $\pm$ 5.0} & 66.8 $\pm$ 5.6 \\
Eye R & \textbf{66.3 $\pm$ 5.3} & 63.4 $\pm$ 5.2 & \textbf{69.5 $\pm$ 4.6} & 67.6 $\pm$ 4.9 \\
Lens L & 22.2 $\pm$ 7.5 & \textbf{16.5 $\pm$ 3.1} & \textbf{21.4 $\pm$ 9.5} & 15.9 $\pm$ 2.8 \\
Lens R & 20.6 $\pm$ 6.9 & \textbf{13.6 $\pm$ 2.8} & \textbf{20.7 $\pm$ 10.8} & 13.8 $\pm$ 3.5 \\
Opt Nerve L & \textbf{31.4 $\pm$ 9.5} & 29.7 $\pm$ 13.2 & \textbf{32.4 $\pm$ 12.9} & 22.2 $\pm$ 17.9 \\
Opt Nerve R & \textbf{34.6 $\pm$ 8.9} & 32.1 $\pm$ 12.2 & 32.2 $\pm$ 15.9 & \textbf{36.4 $\pm$ 13.1} \\
Opt Chiasma & \textbf{29.0 $\pm$ 10.0} & 28.9 $\pm$ 16.0 & \textbf{37.9 $\pm$ 14.9} & 25.3 $\pm$ 14.7 \\
Temporal Lobes L & 25.4 $\pm$ 16.3 & \textbf{72.3 $\pm$ 4.8} & 37.7 $\pm$ 20.2 & \textbf{78.2 $\pm$ 6.4} \\
Temporal Lobes R & 19.9 $\pm$ 20.2 & \textbf{67.7 $\pm$ 8.6} & 34.4 $\pm$ 21.2 & \textbf{76.5 $\pm$ 7.6} \\
Pituitary & \textbf{36.2 $\pm$ 21.1} & 28.5 $\pm$ 16.1 & \textbf{36.6 $\pm$ 17.0} & 29.1 $\pm$ 15.4 \\
Parotid Gland L & 7.1 $\pm$ 6.5 & \textbf{44.2 $\pm$ 10.3} & 27.8 $\pm$ 10.0 & \textbf{50.7 $\pm$ 11.0} \\
Parotid Gland R & 8.1 $\pm$ 8.6 & \textbf{44.7 $\pm$ 8.5} & 30.2 $\pm$ 9.9 & \textbf{49.4 $\pm$ 10.5} \\
Inner Ear L & \textbf{51.7 $\pm$ 16.5} & 48.1 $\pm$ 13.7 & \textbf{56.4 $\pm$ 16.1} & 54.7 $\pm$ 12.4 \\
Inner Ear R & \textbf{63.8 $\pm$ 10.3} & 43.5 $\pm$ 18.8 & \textbf{60.5 $\pm$ 15.8} & 44.5 $\pm$ 16.9 \\
Mid Ear L & \textbf{64.1 $\pm$ 11.8} & 27.7 $\pm$ 14.1 & \textbf{74.4 $\pm$ 7.7} & 39.5 $\pm$ 14.4 \\
Mid Ear R & \textbf{64.7 $\pm$ 10.6} & 33.2 $\pm$ 14.2 & \textbf{74.4 $\pm$ 7.7} & 45.0 $\pm$ 9.6 \\
TM Joint L & \textbf{54.0 $\pm$ 8.3} & 34.9 $\pm$ 12.4 & \textbf{62.8 $\pm$ 11.5} & 37.8 $\pm$ 16.1 \\
TM Joint R & \textbf{58.5 $\pm$ 7.9} & 43.6 $\pm$ 11.1 & \textbf{64.5 $\pm$ 14.8} & 46.6 $\pm$ 11.9 \\
Spinal Cord & \textbf{9.5 $\pm$ 3.8} & 9.4 $\pm$ 3.5 & \textbf{40.4 $\pm$ 6.3} & 32.7 $\pm$ 6.4 \\
Mandible L & \textbf{48.3 $\pm$ 5.1} & 9.0 $\pm$ 3.8 & \textbf{85.3 $\pm$ 2.4} & 11.1 $\pm$ 4.6 \\
Mandible R & \textbf{43.5 $\pm$ 5.3} & 2.6 $\pm$ 2.9 & \textbf{80.4 $\pm$ 2.5} & 12.9 $\pm$ 7.8 \\
\hline
Average          & \textbf{39.6 $\pm$ 7.6} & 37.5 $\pm$ 7.1 & \textbf{50.6 $\pm$ 6.3} & 42.3 $\pm$ 7.8\\ 
\hline
\end{tabular}}
\label{tab:structseg}
\end{table*}

==> tabel/tab5_full.tex <==
\begin{table*}[t!]
    \centering
    \caption{Comparison of segmentation performance between MedLAM-generated bounding box prompts and manually annotated prompts on the StructSeg Head-and-Neck dataset. Metrics include Dice Similarity Coefficient (DSC) and Hausdorff Distance (HD$_{95}$).}
    \textcolor{black}{
    \begin{subtable}{1\textwidth}
    \centering
    \caption{\textcolor{black}{StructSeg Head-and-Neck}}
    \scalebox{0.95}{
    \begin{tabular}{ccccccccc}
    \toprule[1.5pt]
    \multirow{3}*{Organs} & \multicolumn{4}{c}{DSC $\uparrow$ (mean$\pm$std \%)} & \multicolumn{4}{c}{HD$_{95}$ $\downarrow$ (mean$\pm$std mm)} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    ~ &  & \multicolumn{2}{c}{MedLAM} & \multicolumn{2}{c}{Manual Prompt} & \multicolumn{2}{c}{MedLAM} & \multicolumn{2}{c}{Manual Prompt} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    ~ & SAM & MedSAM & SAM & MedSAM & SAM & MedSAM & SAM & MedSAM\\\hline
    Brain Stem       & 63.5$\pm$6.3       & $\bm{73.3\pm5.0}$  & 66.2$\pm$2.7       & $\bm{75.9\pm2.7}$ & 8.4$\pm$1.6       & $\bm{6.2\pm1.2}$  & 8.6$\pm$1.0      & $\bm{6.1\pm1.1}$ \\
    Eye L            & 64.5$\pm$6.5       & $\bm{69.3\pm5.9}$  & 65.7$\pm$5.6       & $\bm{70.0\pm4.6}$ & 8.0$\pm$1.5       & $\bm{5.8\pm1.0}$  & 7.9$\pm$1.3      & $\bm{5.9\pm1.1}$ \\
    Eye R            & 67.3$\pm$5.8       & $\bm{69.4\pm5.5}$  & 68.9$\pm$4.8       & $\bm{69.1\pm5.2}$ & 7.6$\pm$1.9       & $\bm{5.7\pm1.2}$  & 7.4$\pm$1.2      & $\bm{6.2\pm1.1}$ \\
    Lens L           & 15.9$\pm$7.8       & $\bm{16.0\pm6.7}$  & $\bm{22.7\pm5.6}$  & 19.2$\pm$3.5      & $\bm{8.0\pm1.5}$  & 8.6$\pm$1.7       & 10.0$\pm$2.3     & $\bm{9.5\pm1.3}$ \\
    Lens R           & 13.8$\pm$8.8       & $\bm{14.0\pm5.5}$  & $\bm{22.8\pm7.7}$  & 17.3$\pm$4.6      & $\bm{9.3\pm1.5}$  & 9.6$\pm$1.3       & $\bm{9.7\pm2.1}$ & 10.9$\pm$2.3     \\
    Opt Nerve L      & $\bm{23.7\pm6.1}$  & 23.5$\pm$6.2       & 32.6$\pm$9.3       & $\bm{34.7\pm5.4}$ & 9.0$\pm$1.7       & $\bm{8.6\pm1.1}$  & 10.1$\pm$2.5     & $\bm{8.4\pm1.3}$ \\
    Opt Nerve R      & $\bm{27.8\pm10.2}$ & 26.3$\pm$6.6       & 28.5$\pm$6.7       & $\bm{32.4\pm5.2}$ & 9.2$\pm$3.2       & $\bm{9.0\pm1.4}$  & 11.3$\pm$2.2     & $\bm{9.4\pm1.0}$ \\
    Opt Chiasma      & 11.4$\pm$10.6      & $\bm{14.4\pm11.4}$ & 39.8$\pm$10.2      & $\bm{39.8\pm8.1}$ & 10.2$\pm$1.4      & $\bm{8.8\pm1.6}$  & 7.2$\pm$1.7      & $\bm{6.6\pm1.2}$ \\
    Temporal Lobes L & 28.2$\pm$15.2      & $\bm{78.3\pm3.5}$  & 36.8$\pm$16.6      & $\bm{83.5\pm1.9}$ & 16.4$\pm$3.5      & $\bm{9.0\pm2.1}$  & 13.7$\pm$3.5     & $\bm{6.6\pm1.4}$ \\
    Temporal Lobes R & 24.1$\pm$17.4      & $\bm{78.0\pm4.3}$  & 30.7$\pm$17.8      & $\bm{84.4\pm1.4}$ & 18.2$\pm$4.2      & $\bm{10.1\pm2.4}$ & 15.1$\pm$4.1     & $\bm{6.1\pm2.5}$ \\
    Pituitary        & $\bm{12.5\pm10.7}$ & 10.2$\pm$9.2       & $\bm{36.6\pm16.2}$ & 27.5$\pm$12.5     & $\bm{8.7\pm2.2}$  & 8.8$\pm$1.8       & $\bm{7.4\pm2.0}$ & 10.0$\pm$3.6     \\
    Parotid Gland L  & 15.5$\pm$11.9      & $\bm{59.6\pm6.5}$  & 29.5$\pm$7.7       & $\bm{64.4\pm3.4}$ & 17.6$\pm$3.0      & $\bm{10.3\pm1.9}$ & 16.0$\pm$1.9     & $\bm{9.3\pm1.9}$ \\
    Parotid Gland R  & 17.2$\pm$9.9       & $\bm{57.1\pm6.8}$  & 29.6$\pm$6.5       & $\bm{64.9\pm5.0}$ & 19.8$\pm$5.0      & $\bm{13.5\pm3.5}$ & 14.0$\pm$2.1     & $\bm{9.5\pm1.6}$ \\
    Inner Ear L      & 40.4$\pm$11.8      & $\bm{42.3\pm9.9}$  & 59.7$\pm$11.7      & $\bm{62.1\pm9.7}$ & 9.4$\pm$1.7       & $\bm{7.6\pm1.5}$  & 7.6$\pm$2.1      & $\bm{5.9\pm1.8}$ \\
    Inner Ear R      & $\bm{48.9\pm9.5}$  & 45.9$\pm$11.2      & $\bm{67.3\pm10.4}$ & 66.9$\pm$6.1      & 8.4$\pm$1.7       & $\bm{7.0\pm1.7}$  & 6.8$\pm$1.9      & $\bm{5.4\pm1.2}$ \\
    Mid Ear L        & $\bm{64.6\pm14.3}$ & 59.7$\pm$9.6       & $\bm{71.0\pm11.7}$ & 67.5$\pm$6.3      & 7.9$\pm$2.6       & $\bm{7.7\pm1.6}$  & 6.4$\pm$2.8      & $\bm{6.1\pm1.1}$ \\
    Mid Ear R        & $\bm{64.7\pm13.1}$ & 59.3$\pm$11.2      & $\bm{73.3\pm7.7}$  & 65.0$\pm$8.9      & 8.4$\pm$2.4       & $\bm{7.6\pm1.4}$  & $\bm{6.2\pm1.9}$ & 6.6$\pm$1.2      \\
    TM Joint L       & 38.3$\pm$10.1      & $\bm{39.0\pm10.9}$ & 59.7$\pm$12.8      & $\bm{61.2\pm4.9}$ & 10.2$\pm$2.1      & $\bm{7.7\pm1.6}$  & 6.8$\pm$1.9      & $\bm{6.0\pm0.7}$ \\
    TM Joint R       & $\bm{41.5\pm10.0}$ & 38.3$\pm$9.5       & 59.2$\pm$17.8      & $\bm{60.0\pm7.7}$ & 9.6$\pm$1.6       & $\bm{8.1\pm1.4}$  & 8.2$\pm$1.9      & $\bm{6.3\pm1.1}$ \\
    Spinal Cord      & 27.9$\pm$8.3       & $\bm{34.7\pm6.9}$  & 38.0$\pm$7.7       & $\bm{40.3\pm6.1}$ & 15.5$\pm$2.7      & $\bm{13.3\pm2.9}$ & 10.7$\pm$1.3     & $\bm{8.8\pm0.9}$ \\
    Mandible L       & $\bm{78.0\pm4.9}$  & 66.7$\pm$6.1       & $\bm{86.0\pm2.1}$  & 76.8$\pm$4.7      & $\bm{11.1\pm2.8}$ & 11.8$\pm2.1$      & $\bm{5.5\pm1.7}$ & 9.0$\pm$4.5      \\
    Mandible R       & $\bm{71.4\pm4.0}$  & 66.0$\pm$4.7       & $\bm{81.2\pm2.7}$  & 75.0$\pm$4.5      & 22.6$\pm$4.7      & $\bm{12.3\pm2.6}$ & 21.6$\pm$5.4     & $\bm{9.6\pm3.5}$ \\ \hline
    Average          & 39.1$\pm$9.7       & $\bm{47.3\pm7.4}$ & 50.3$\pm$9.2       & $\bm{57.2\pm5.6}$ & 11.5$\pm$2.5      & $\bm{9.0\pm1.8}$  & 9.9$\pm$2.2      & $\bm{7.6\pm1.7}$ \\ 
    \bottomrule[1.5pt]
    \end{tabular}}
    \end{subtable}}
    
    \vspace{0.2cm}
    
    \textcolor{black}{
    \begin{subtable}{1\textwidth}
    \centering
    \caption{\textcolor{black}{WORD}}
    \scalebox{0.95}{
    \begin{tabular}{ccccccccc} \bottomrule[1.5pt]
    \multirow{3}*{Organs} & \multicolumn{4}{c}{DSC $\uparrow$ (mean$\pm$std \%)} & \multicolumn{4}{c}{HD$_{9}$ $\downarrow$ (mean$\pm$std mm)} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    ~ & \multicolumn{2}{c}{MedLAM} & \multicolumn{2}{c}{Manual Prompt} & \multicolumn{2}{c}{MedLAM} & \multicolumn{2}{c}{Manual Prompt} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    ~ & SAM & MedSAM & SAM & MedSAM & SAM & MedSAM & SAM & MedSAM\\\hline
    Liver           & $\bm{66.0\pm10.1}$ & 23.8$\pm$8.6      & $\bm{84.2\pm6.3}$  & 46.6$\pm$14.7     & 53.6$\pm$10.4       & $\bm{51.5\pm8.6}$  & $\bm{21.8\pm11.9}$ & 36.8$\pm$11.6      \\
    Spleen          & $\bm{61.7\pm14.4}$ & 36.3$\pm$13.2     & $\bm{85.3\pm5.1}$  & 65.0$\pm$6.3      & $\bm{30.1\pm16.1}$  & 30.5$\pm$14.4      & $\bm{10.8\pm6.5}$  & 16.2$\pm$4.9       \\
    Kidney L        & $\bm{82.1\pm16.0}$ & 70.7$\pm$18.8     & $\bm{92.1\pm1.6}$  & 84.1$\pm$5.2      & 19.2$\pm$18.6       & $\bm{18.5\pm16.9}$ & $\bm{6.1\pm1.9}$   & 8.2$\pm$1.6        \\
    Kidney R        & $\bm{88.3\pm4.8}$  & 77.3$\pm$6.2      & $\bm{92.9\pm1.6}$  & 86.4$\pm$3.1      & $\bm{12.7\pm5.7}$   & 13.4$\pm$4.1       & $\bm{6.0\pm1.6}$   & 7.7$\pm$1.2        \\
    Stomach         & $\bm{44.6\pm15.0}$ & 37.2$\pm$14.7     & 77.1$\pm$10.6      & $\bm{80.3\pm4.7}$ & $\bm{50.1\pm27.0}$  & 51.7$\pm$27.6      & 12.7$\pm$4.2       & $\bm{11.5\pm3.6}$  \\
    Gallbladder     & $\bm{13.1\pm17.3}$ & 10.2$\pm$13.4     & $\bm{72.7\pm11.1}$ & 68.8$\pm$7.8      & 36.8$\pm$19.8       & $\bm{36.7\pm20.4}$ & $\bm{6.0\pm1.8}$   & 6.4$\pm$1.6        \\
    Esophagus       & $\bm{36.6\pm14.7}$ & 27.8$\pm$12.9     & $\bm{67.0\pm6.4}$  & 63.1$\pm$7.7      & 21.1$\pm$12.7       & $\bm{19.8\pm11.6}$ & 6.9$\pm$4.0        & $\bm{6.7\pm3.2}$   \\
    Pancreas        & $\bm{29.7\pm14.1}$ & 21.4$\pm$9.7      & $\bm{64.4\pm7.7}$  & 46.9$\pm$11.6     & $\bm{32.6\pm13.5}$  & 33.1$\pm$10.8      & $\bm{15.9\pm6.4}$  & 18.3$\pm$5.5       \\
    Duodenum        & $\bm{26.0\pm11.4}$ & 21.1$\pm$7.0      & $\bm{54.1\pm13.2}$ & 51.0$\pm$11.9     & 31.1$\pm$9.7        & $\bm{30.9\pm10.4}$ & $\bm{16.0\pm4.6}$  & 17.1$\pm$5.9       \\
    Colon           & 25.6$\pm$9.6       & $\bm{26.6\pm8.9}$ & 41.8$\pm$6.8       & $\bm{44.1\pm8.8}$ & $\bm{57.8\pm17.8}$  & 60.6$\pm$17.8      & 49.4$\pm$15.3      & $\bm{49.1\pm13.9}$ \\
    Intestine       & $\bm{37.5\pm7.6}$  & 34.1$\pm$8.4      & $\bm{61.4\pm6.9}$  & 52.5$\pm$8.0      & 47.1$\pm$10.5       & $\bm{44.1\pm10.0}$ & 21.7$\pm$4.2       & $\bm{21.0\pm4.0}$  \\
    Adrenal         & 3.3$\pm$3.9        & $\bm{10.0\pm6.2}$ & 17.4$\pm$8.8       & $\bm{26.5\pm5.9}$ & 30.8$\pm$8.7        & $\bm{29.9\pm7.5}$  & 23.4$\pm$4.3       & $\bm{22.6\pm2.7}$  \\
    Rectum          & $\bm{50.1\pm17.9}$ & 46.0$\pm$18.7     & 75.5$\pm$4.0       & $\bm{80.0\pm3.6}$ & 18.6$\pm$7.0        & $\bm{17.4\pm7.2}$  & 7.6$\pm$0.9        & $\bm{4.8\pm0.6}$   \\
    Bladder         & $\bm{65.3\pm26.6}$ & 59.1$\pm$23.1     & $\bm{83.0\pm15.5}$ & 82.9$\pm$8.0      & 20.5$\pm$10.2       & $\bm{19.8\pm8.8}$  & 7.5$\pm$3.5        & $\bm{6.9\pm2.0}$   \\
    Head of Femur L & $\bm{81.7\pm3.9}$  & 71.5$\pm$4.1      & $\bm{90.5\pm2.7}$  & 80.3$\pm$2.8      & 16.6$\pm$3.3        & $\bm{14.9\pm1.6}$  & $\bm{9.2\pm4.7}$   & 12.3$\pm$2.0       \\
    Head of Femur R & $\bm{80.1\pm3.3}$  & 74.3$\pm$4.4      & $\bm{89.1\pm3.4}$  & 83.2$\pm$2.7      & 19.5$\pm$2.6        & $\bm{13.4\pm1.0}$  & 12.6$\pm$6.1       & $\bm{12.3\pm7.7}$  \\ \hline
    Average         & $\bm{49.5\pm11.9}$ & 40.5$\pm$11.1     & $\bm{71.8\pm7.0}$  & 65.1$\pm$7.0      & 31.1$\pm$12.1       & $\bm{30.4\pm11.2}$ & $\bm{14.6\pm5.1}$  & 16.1$\pm$4.5       \\
    \bottomrule[1.5pt]
    \end{tabular}}
    \end{subtable}
    }
    \label{tab:4}
    \end{table*}

==> tabel/word.tex <==
\begin{table*}[!h]
\caption{DSC (mean$\pm$std \%) evaluation of 3D abdomen organs segmentation in the WORD dataset. The table compares the performance of SAM and MedSAM as segmentation basis within the MedLSAM framework, along with results from manually assisted localizations.}
\centering
\begin{tabular}{c|cc|cc} \hline
Localization & \multicolumn{2}{c|}{MedLAM} & \multicolumn{2}{c}{Manual} \\ \cline{1-5}
Organs & SAM & MedSAM & SAM & MedSAM\\\hline
Liver & 55.5 $\pm$ 9.5 & \textbf{67.1 $\pm$ 8.7} & \textbf{84.5 $\pm$ 6.3} & 76.3 $\pm$ 6.7 \\
Spleen & \textbf{60.9 $\pm$ 12.4} & 40.3 $\pm$ 20.8 & \textbf{87.2 $\pm$ 7.3} & 60.2 $\pm$ 19.4 \\
Kidney L & \textbf{78.5 $\pm$ 12.1} & 66.2 $\pm$ 13.1 & \textbf{92.0 $\pm$ 4.4} & 72.3 $\pm$ 7.3 \\
Kidney R & \textbf{83.0 $\pm$ 11.0} & 62.3 $\pm$ 9.7 & \textbf{92.9 $\pm$ 2.3} & 67.1 $\pm$ 6.7 \\
Stomach & \textbf{43.0 $\pm$ 13.1} & 35.2 $\pm$ 15.9 & \textbf{79.4 $\pm$ 8.6} & 62.2 $\pm$ 14.6 \\
Gallbladder & \textbf{33.2 $\pm$ 25.0} & 27.8 $\pm$ 22.7 & \textbf{72.9 $\pm$ 9.7} & 67.3 $\pm$ 10.5 \\
Esophagus & \textbf{24.6 $\pm$ 11.2} & 22.1 $\pm$ 13.8 & \textbf{68.2 $\pm$ 6.8} & 48.2 $\pm$ 13.5 \\
Pancreas & \textbf{34.1 $\pm$ 12.1} & 28.4 $\pm$ 11.0 & \textbf{64.0 $\pm$ 11.8} & 56.7 $\pm$ 9.2 \\
Duodenum & \textbf{22.9 $\pm$ 13.2} & 18.5 $\pm$ 9.8 & \textbf{59.7 $\pm$ 11.9} & 42.3 $\pm$ 11.3 \\
Colon & \textbf{18.5 $\pm$ 6.3} & 12.8 $\pm$ 8.3 & \textbf{42.9 $\pm$ 9.0} & 22.0 $\pm$ 9.9 \\
Intestine & \textbf{35.5 $\pm$ 9.3} & 20.2 $\pm$ 8.8 & \textbf{60.2 $\pm$ 7.2} & 31.3 $\pm$ 9.1 \\
Adrenal & \textbf{3.8 $\pm$ 5.2} & 3.4 $\pm$ 3.1 & \textbf{18.7 $\pm$ 12.1} & 17.3 $\pm$ 10.0 \\
Rectum & \textbf{37.6 $\pm$ 11.1} & 29.9 $\pm$ 12.9 & \textbf{74.4 $\pm$ 5.5} & 53.7 $\pm$ 12.9 \\
Bladder & \textbf{68.4 $\pm$ 21.3} & 62.4 $\pm$ 17.8 & \textbf{85.8 $\pm$ 11.6} & 73.7 $\pm$ 10.5 \\
Head of Femur L & \textbf{74.5 $\pm$ 7.7} & 48.2 $\pm$ 15.6 & \textbf{89.3 $\pm$ 4.7} & 62.1 $\pm$ 12.8 \\
Head of Femur R & \textbf{71.5 $\pm$ 5.3} & 46.6 $\pm$ 10.1 & \textbf{87.9 $\pm$ 3.6} & 65.5 $\pm$ 7.0 \\
\hline
Average & \textbf{45.9 $\pm$ 11.2} & 37.7 $\pm$ 12.4 & \textbf{72.5 $\pm$ 3.1} & 54.9 $\pm$ 6.7\\
\hline
\end{tabular}
\label{tab:word}
\end{table*}
